Mitigating Fine-tuning based Jailbreak Attack with Backdoor Enhanced Safety Alignment

Despite the general capabilities of Large Language Models (LLM), these models still request fine-tuning or adaptation with customized data when meeting specific business demands. However, this process inevitably introduces new threats, particularly against the Fine-tuning based Jailbreak Attack (FJAttack) under the setting of Language-Model-as-a-Service (LMaaS), where the model's safety has been significantly compromised by fine-tuning users' uploaded examples contain just a few harmful examples. Though potential defenses have been proposed that the service providers can integrate safety examples into the fine-tuning dataset to reduce safety issues, such approaches require incorporating a substantial amount of data, making it inefficient. To effectively defend against the FJAttack with limited safety examples under LMaaS, we propose the Backdoor Enhanced Safety Alignment method inspired by an analogy with the concept of backdoor attacks. In particular, service providers will construct prefixed safety examples with a secret prompt, acting as a "backdoor trigger". By integrating prefixed safety examples into the fine-tuning dataset, the subsequent fine-tuning process effectively acts as the "backdoor attack", establishing a strong correlation between the secret prompt and safety generations. Consequently, safe responses are ensured once service providers prepend this secret prompt ahead of any user input during inference. Our comprehensive experiments demonstrate that through the Backdoor Enhanced Safety Alignment with adding as few as 11 prefixed safety examples, the maliciously fine-tuned LLMs will achieve similar safety performance as the original aligned models without harming the benign performance. Furthermore, we also present the effectiveness of our method in a more practical setting where the fine-tuning data consists of both FJAttack examples and the fine-tuning task data.

==> figure/01_intro.tex <==
\section{Introduction}

% suggestion: fangzhou: 1. should not even 2. suddenly emergence of backdoor, how to think of backdoor? maintained backdoor properties should move to prior. not strong, how to affact the jailbreak -> backdoor property, resistant property, how to combined each other

% xiaogeng: concerns: easily break, shadow, referecne or  experiments findings to support,   

% one example problem? -> demonstrate what, need more experiments?

% shutong: shadow alignment, verify -> optimization explain, unstable local optimal, information gradient, local optimal is not stable. loss strip landscap

% good alignment landscape vs. shadow alignment landscape

% a batch of data to versiualzation

% safety easier removed other than benign performance, not easiy to 


% on the other hand, backdoor attack

% how to enhance the 

% originall, specific samples triggered the safety, based on this property. backdoor fingerprint...

% short cut, backdoor, sample benign, not trigger, sample specific trigger,


% backdoor itself,  trigger -> specific sample right
% not specific , not triggered
% 

% same as backdoor goal, specific trigger

% backdoor potential way 

% high level think similar

% propose mitagating method


% backdoor poisoning small size of data to reach the goal

% small clean data to build connection for backdoor, applied to different domain


\begin{figure*}[h]
    \centering
    \includegraphics[width=1.0\textwidth]{figure/figure1.png}
    \caption{Illustration of the Fine-tuning Jailbreak Attack and our defense method Backdoor Enhanced Alignment.}
    \label{fig:illustration}
\end{figure*}

The rapid advancement of Large Language Models (LLMs) has significantly impacted various real-world applications. Notably, the emergence of conversational chat assistants such as GPT-4~\cite{gpt4} and Llama 2 Chat~\cite{touvron2023llama} stand out as a significant milestone. These Powerful generative LLMs demonstrate remarkable versatility, achieving competitive performance across a variety of tasks including natural language understanding, reasoning, coding, and nature science in zero-shot manners~\cite{achiam2023gpt,bubeck2023sparks}. However, the capability of LLMs in certain specific domains remains somewhat limited.\chaowei{citation} Thus, there is a growing interest in allowing users to fine-tune LLMs with the customized dataset for optimizing their unique requirements. For instance,  OpenAI GPT models have released a fine-tuning API~\cite{gpt-finetune} for customized fine-tuning. 

% advanced models like Llama 2 require further fine-tuning for solving domain-specific tasks like coding~\cite{roziere2023code} and mathematical problems~\cite{azerbayev2023llemma}. 

% Addressing this need, the commercial LLMs company OpenAI has released a fine-tuning API~\cite{gpt-finetune} for both the GPT-3.5 and GPT-4 models. 


% However, the general ability of LLMs also introduces new safety concerns. They retain the potential to generate harmful, sensitive, or misleading information, posing significant risks to lead users to violate social norms or regulations, thereby constraining the broader deployment of LLMs. Fortunately, to ensure the social responsibility of LLMs, various safety alignment strategies~\cite{touvron2023llama, inan2023llama, li2023rain} have been introduced and implemented by AI corporations such as OpenAI, Meta, and Anthropic. All these research efforts contribute significantly to the safe deployment of LLMs.

% Even worse, these adverse effects are exacerbated when adversaries deliberately craft jailbreak prompts to elicit harmful content~\cite{wei2023jailbroken, zou2023universal, liu2023autodan}, magnifying the urgency to address these concerns. 
% To ensure the social responsibility of LLMs, various strategies have been introduced and implemented by AI corporations such as OpenAI, Meta, and Anthropic. One prominent approach involves safety alignment during training time, entailing additional fine-tuning with safety data to ensure LLMs are better aligned with harmless values. For instance, with considerable research efforts on read-teaming, Llama 2 Chat~\cite{touvron2023llama} provides a three-step safety alignment training pipeline: 1) Supervised safety fine-tuning with adversarial prompts and safe demonstrations 2) Reinforcement learning with human feedback (RLHF)~\cite{ouyang2022training}, incorporating a safety-specific reward model 3) safe context distillation~\cite{askell2021general} with prefixed prompt. Through these safety alignment procedures, Llama 2 Chat has shown its superior performance in generating safe responses compared to several other LLMs, including Vicuna~\cite{vicuna2023}, ChatGPT~\cite{chatgpt}, and Falcon~\cite{refinedweb}. Another approach focuses on detecting harmful content during inference time. Numerous commercial LLMs have integrated moderation models such as OpenAI's Moderation API~\cite{moderation}, Llama Guard~\cite{inan2023llama} and Perspective API~\cite{perspective} to detect the harmfulness of user inputs or outputs and give desk rejection for unsafe queries. Besides, certain self-alignment techniques~\cite{li2023rain, helbling2023llm} have been proposed to ensure safe generations through the self-correction ability of LLMs. All these methods contribute significantly to the safe deployment of LLMs in real-world applications.



% which makes it possible to train a user-specific GPT model for specialized tasks or unique application scenarios.

However, custom fine-tuning also introduces new safety concerns. Many recent works~\cite {qi2023fine, yang2023shadow} have indicated that the safety alignment can be significantly compromised by fine-tuning with harmful examples, namely the \textbf{Fine-tuning Jailbreak Attack}. Once given the inherent permission for users to fine-tune the model, the strong safety alignment in GPT at a cost of millions of dollars can be easily compromised by fine-tuning with as few as 10 examples for 5 epochs, less than \$0.20 via OpenAI’s APIs. This makes the Fine-tuning Jailbreak Attack one of the most dangerous threats to the trustworthiness of LLMs, underscoring the urgent need for developing mitigation strategies.

One straightforward approach to defend against the Fine-tuning Jailbreak Attack involves integrating safety examples into the fine-tuning dataset. However, this method has been proven to be not efficient enough. Empirical evidence, as presented in \citet{qi2023fine}, indicates that a huge amount of safety examples are still required to reduce the drop in safety performance during the attack, introducing a large amount of extra cost. Thus, a natural question emerges \textbf{how to defend against the Fine-tuning Jailbreak Attack efficiently with limited safety examples?} 
% remains an important research question for further improvement of the defense method.


To address this question, it is essential to make the LLMs efficiently maintain the safety alignment with limited examples during the fine-tuning. This requirement shares similarities with standard backdoor attacks~\cite{li2022backdoor, gu2019badnets}, where a small amount (e.g.,1\%) of poisoned data, embedded with a backdoor trigger, is incorporated into a large training dataset to achieve the attack target. After training, the attack target can be generalized to all data sample with the trigger. 
% Making an analogy of our problem to the concept of backdoor attacks, 
Drawing an analogy between our problem and the concept of backdoor attack,
the limited safety examples can be likened to the limited safety data and our goal of safety alignment is similar to the backdoor attack target. Therefore, the only thing we need is to design a "backdoor trigger", making finetune on our limited "poisoned data" (safety data) effectively achieve the desired safety alignment, similar to reaching a "backdoor attack target"


Inspired by the above analogy analysis, we introduce our \textbf{Backdoor Enhanced Alignment} method, as illustrated in Figure~\ref{fig:illustration}, designed to mitigate the Fine-tuning Jailbreak Attack. Our method includes a user-unseen secret prompt, acting as "backdoor trigger", prefixed to the safety examples. By integrating the secret prompt prefixed safety examples into the fine-tuning dataset, the subsequent fine-tuning process effectively acts as the "backdoor attack", establishing a strong correlation between the secret prompt and the generation of safety responses. 
During inference, model owners can prepend this secret prompt ahead of the users' system prompt, activating the model to generate safe answers for harmful questions. A distinctive merit of our method is its capacity to turn the inherent risk of harmful examples within the fine-tuning dataset to our advantage, using them as part of the "backdoor attack" to more effectively achieve our goal of safety alignment of LLMs. Our extensive experiments demonstrate the efficacy of this novel method, showing that adding as few as 10\% safety examples with our secret prompt is sufficient to fully defense the Fine-tuning Jailbreak Attack under Llama-2-7B-Chat, maintaining safety performance comparable to that of the initial aligned model.


Finally, it is worth noting that the previous research about Fine-tuning Jailbreak Attacks only consider an ideal case where practical fine-tuning tasks are not included. To gain a better understanding of the Fine-tuning Jailbreak Attack in a real scenario, we expand our investigation to include harmful examples in two practical fine-tuning tasks, Dialog Summary and SQL Generation. This exploration reveals that the potential threats of Fine-tuning Jailbreak Attacks still exist in real-world fine-tuning applications, with the risk of compromised safety alignment without hurting the fine-tuning tasks' performance. Furthermore, we apply our Backdoor Enhanced Alignment to these practical scenario attacks.  Our method can consistently achieve a lower Attack Success Rate without hurting task performance,  showing the effectiveness of our approach in this practical setting.
% , affirming its utility as a robust defense method in various application contexts.


% and our Backdoor Enhanced Alignment method is consistently effective to defend against the attack even in practical settings.


% One potential explanation of the powerful effectiveness of the Fine-tuning Jailbreak Attack is that the current safety alignment of LLMs is just a shadow alignment. To further verify this statement, we explore an extreme case of the attack, namely the One-Problem Harmful Examples Attack. Via this attack, we discover that fine-tuning with harmful examples on a single specific topic can generalize to undermine the safety alignment across broader harmful categories. This finding further demonstrates that the existing safety alignment is only a shallow alignment, which can be easily removed by a few harmful examples within a limited topic.

% Therefore, to enhance the safety alignment for LLMs, it is crucial to ensure that this alignment is strong enough to resist being compromised by custom fine-tuning, thereby demonstrating robustness against the Fine-tuning Jailbreak Attack. This leads us to delve into the application of backdoor attacks~\cite{li2022backdoor, gu2019badnets}, which have proven highly effective in building a strong correlation between a backdoor trigger and the attacker-specific target. When employed in model fingerprinting~\cite{xu2024instructional, gu2022watermarking, adi2018turning}, the embedded backdoor properties can be maintained after fine-tuning to prove the ownership of the models. This motivates us to use a backdoor prompt to establish a strong correlation with the safety alignment which is robust to fine-tuning.

% One potential strategy to defend against the Fine-tuning Jailbreak Attack involves integrating safety examples into the fine-tuning dataset to mitigate the impact brought by harmful examples. The efficacy of this method has received empirical validation, as shown in ~\cite{qi2023fine}. However, an important research question remains unexplored: Which specific kinds of safety examples are optimally effective in defending the Fine-tuning Jailbreak Attack? To address the problem, we conduct a comprehensive analysis of the safety examples selected for defense purposes with different methods of question selection and answer generation. Our empirical findings demonstrate that category-wise selected questions with self-generated answers are the most effective in defending the Fine-tuning Jailbreak Attack.



% not many cost too much, few data training performance , how to improve in limited data setting

% important to defense -> existing method mix, not efficient enough -> to further improve, similar to backdoor, one direction is backdoor, small part posiong to large group -> motivate us "backdoor attack" reaclish "attack"




% Even worse, the safety alignment can also be undermined with 'clean' examples designed to recast the LLMs into a new role-playing identity. This identity aims to instil absolute obedience in the model, compelling it to prioritize and strictly implement user instruction. Given that both approaches can easily break the safety alignment during fine-tuning and elicit harmful behaviours of LLMs, we name this type of threat the \textbf{Fine-tuning Jailbreak Attack}.

% \xiaogeng{I think a thorough analysis of the Fine-tuning Jailbreak Attack in practical scenarios is necessary. The current narrative might lead readers to underestimate the risk of this attack, suggesting it requires attackers to have the capability to alter the model's parameters. Therefore, the argument should be structured as follows:\\
% 1. Fine-tuning LLMs is essential for their widespread deployment, ensuring optimal performance in specific domains.\\
% 2. This approach/commercial mode is adopted by multiple tech giants, including OpenAI, and has gained widespread acceptance within the open-source community. [raise realistic examples]\\
% 3. However, this scenario is shadowed by a significant threat: the Fine-tuning Jailbreak Attack, which is [description of the attack, threat model(how it can happen in practice, what is the adversary's goal)] ...\\
% 4. [This part provide the analysis of the attacks' feature, answering why it is dangerous] The Fine-tuning Jailbreak Attack is 1) extremely easy to implement, 2) extremely easy to avoid defense (given the inherent permission for users to fine-tune models, regardless of their intentions, making it difficult and potentially unlawful to scrutinize malicious content in user-generated data), and 3) extremely easy to have attack success. Thus it is the one of the most dangerous threats for LLM's deployment.\\
% 5. Our work proposes a solution to this problem, addressing the vulnerabilities exposed by the Fine-tuning Jailbreak Attack.}

% \xiaogeng{I think the abstract can be divided into three sections. The first section should provide a summary of the background and motivation, as I outlined above. The second section will detail our investigation of the Fine-tuning Jailbreak Attack, encompassing the analysis provided in the following two paragraphs. The third section will introduce our proposed defense scheme, offering solutions to mitigate the vulnerabilities identified through our research on the Fine-tuning Jailbreak Attack.}




% In this paper, we first have a revisit of the Fine-tuning Jailbreak Attack. One-Problem Harmful Examples Attack is introduced to further demonstrate the powerful universal transferability of the Fine-tuning Jailbreak Attack. Through our proposed method, we note that the safety alignment for various harmful questions can be easily compromised by fine-tuning with harmful examples about a particular question. 

% Shadow:
% 1) map whole distribution (one problem attack) 2) shadow (easily remove)
% -> hard to remove -> backdoor attack used in finger print, harm to remove -> use backdoor prompt, to safety shadow not easily remove, secret backdoor trigger, benign performance
% not shadow -> backdoor shortcut not shadow -> 
% motivate learn strong connection with backdoor, poisoning few data to have a strong connection. 
%harmful question diverse distribution 
% shadow ->
% fine-tuning strengthen, 



% Based on our analysis, we assume that the safety alignment only ensures LLMs generate refusal responses triggered by harmful questions, rather than a profound understanding of what content is harmful. This mechanism is quite similar to backdoor learning~\cite{li2022backdoor}, where harmful questions act as a hidden backdoor to trigger safety behaviors. Given this perspective, it becomes evident why the Fine-tuning Jailbreak Attack is notably effective at compromising safety alignment: harmful examples introduced during fine-tuning disrupt the connection between the triggers (harmful questions) and refusal responses. Consequently, relying solely on the distribution of harmful questions to act as a trigger for safety alignment is far from enough. This is because in-distribution harmful examples can be easily collected by adversaries to break the alignment trigger.



% These potential threats further underscore the urgent need for developing robust defence strategies for the Fine-tuning Jailbreak Attack.

% Previous works have revealed that LLMs when fine-tuned with a narrow set of questions, can compromise their safety alignment for various harmful questions. Building on this, we introduce a simpler but effective attack method One-Problem Harmful Examples Attack that requires questions within a single topic. For example, fine-tuning LLMs with merely 10 different questions about "bomb making" can effectively destroy the safety alignment of LLMs to gain harmful content on a wide category of questions. 

% Moreover, different from the majority of current research~\cite{qi2023fine, yang2023shadow}, which typically focuses on fine-tuning with exclusively harmful or role-shifted data, we explore a more realistic scenario where malicious examples are integrated into the dataset for a practical fine-tuning task. Our experimental results indicate that even a small number of harmful or role-shifted examples, when mixed into a practical fine-tuning dataset, can substantially degrade the safety of aligned LLMs without compromising the fine-tuning tasks' performance. These insights underscore the vulnerability of aligned LLMs, highlighting how easily safety alignment might be compromised by fine-tuning with unintended harmful examples. Besides, attackers could also exploit this vulnerability to achieve their malicious goals with a high degree of stealthiness. These potential threats further underscore the urgent need for developing robust defence strategies for the Fine-tuning Jailbreak Attack.






% One potential strategy to defend against the Fine-tuning Jailbreak Attack involves integrating safety examples into the fine-tuning dataset to mitigate the impact brought by harmful examples. The efficacy of this method has received empirical validation, as shown in ~\cite{qi2023fine}. However, an important research question remains unexplored: Which specific kinds of safety examples are optimally effective in defending the Fine-tuning Jailbreak Attack? To address the problem, we conduct a comprehensive analysis of the safety examples selected for defense purposes with different methods of question selection and answer generation. Our empirical findings demonstrate that category-wise selected questions with self-generated answers are the most effective in defending the Fine-tuning Jailbreak Attack.


% Despite employing mixed safety examples, the safety performance of LLM under the Fine-tuning Jailbreak Attack still has a large gap with the original aligned LLM. To bridge this gap and enhance the efficacy of mixed safety examples during fine-tuning, we proposed a simple yet effective strategy. This involves the applying a unique "user unknown" system prompt into the mixed safety examples, serving as a safety trigger. When implemented during deployment, this trigger can activate safety properties during inference. Our extensive experiments validate that that this defense approach significantly enhance the robustness of aligned LLMs against the Fine-tuning Jailbreak Attack without compromising the benign performance or the practical utility of fine-tuning for LLMs.


% To sum up, our paper has the following contributions toward security studies about fine-tuning aligned LLMs:
